MotionLLM: Understanding Human Behaviors from Human Motions and Videos

This study delves into the realm of multi-modality (i.e., video and motion modalities) human behavior understanding by leveraging the powerful capabilities of Large Language Models (LLMs). Diverging from recent LLMs designed for video-only or motion-only understanding, we argue that understanding human behavior necessitates joint modeling from both videos and motion sequences (e.g., SMPL sequences) to capture nuanced body part dynamics and semantics effectively. In light of this, we present MotionLLM, a straightforward yet effective framework for human motion understanding, captioning, and reasoning. Specifically, MotionLLM adopts a unified video-motion training strategy that leverages the complementary advantages of existing coarse video-text data and fine-grained motion-text data to glean rich spatial-temporal insights. Furthermore, we collect a substantial dataset, MoVid, comprising diverse videos, motions, captions, and instructions. Additionally, we propose the MoVid-Bench, with carefully manual annotations, for better evaluation of human behavior understanding on video and motion. Extensive experiments show the superiority of MotionLLM in the caption, spatial-temporal comprehension, and reasoning ability.

==> section/limitation.tex <==
\section*{Limitation and Impact Statement}

Although MotionLLM shows good performance on existing and our benchmarks, we still witness a bottleneck in the capacity of visual encoders, which restricts the understanding ability of the model. We leave the development of better visual encoders as our future work. Our work has several social impacts. MotionLLM promises to serve as an AI assistant in many scenarios, like a fitness coach for social goods, especially for the visually impaired community. For the negative part, the development of LLMs might raise the possibility of negative use of our model, such as generating misleading or negative content on social media. 
